Optimization using Parallel Gradient Evaluations on Multiple Parameters

We propose a first-order method for convex optimization, where instead of being restricted to the gradient from a single parameter, gradients from multiple parameters can be used during each step of gradient descent. This setup is particularly useful when a few processors are available that can be used in parallel for optimization. Our method uses gradients from multiple parameters in synergy to update these parameters together towards the optima. While doing so, it is ensured that the computational and memory complexity is of the same order as that of gradient descent. Empirical results demonstrate that even using gradients from as low as \textit{two} parameters, our method can often obtain significant acceleration and provide robustness to hyper-parameter settings. We remark that the primary goal of this work is less theoretical, and is instead aimed at exploring the understudied case of using multiple gradients during each step of optimization.

==> (arXiv) Optimization using Parallel Gradient Evaluations on Multiple Parameters/opt_header.tex <==
% Get better typography
% \usepackage[protrusion=true,expansion=true]{microtype}		

% Small margins
%\usepackage[top=2cm, bottom=2cm, left = 1cm, right = 1cm,columnsep=20pt]{geometry}


% For basic math, align, fonts, etc.
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{dsfont}
% \usepackage[scr=esstix,cal=boondox]{mathalfa} 

\usepackage{courier} % For \texttt{foo} to put foo in Courier (for code / variables)

\usepackage{lipsum} % For dummy text
% Table of contents
\usepackage{etoc}

% for underlining text

\def\mul#1#2{\color{#1}\underline{{\color{black}#2}}\color{black}}
% \usepackage{soul} 
% \newcommand{\myul}[2][black]{\setulcolor{#1}\ul{#2}\setulcolor{black}}

% For images
% \usepackage{graphicx}
% \usepackage{subcaption}
\usepackage[space]{grffile} % For spaces in image names
\usepackage{cancel} % For diagonally striking out equations
\usepackage{tablefootnote}

% For bibliography
% \usepackage[numbers]{natbib}
\usepackage{natbib}


% For links (e.g., clicking a reference takes you to the phy)
\usepackage{hyperref}

% For color
% \usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\definecolor{dark-red}{rgb}{0.4,0.15,0.15}
\definecolor{dark-blue}{rgb}{0,0,0.7}
\hypersetup{
    colorlinks, linkcolor={dark-blue},
    citecolor={dark-blue}, urlcolor={dark-blue}
}


% Macros
\newcommand{\yash}[1]{\textcolor{blue}{[#1---yash]}}
\newcommand{\imp}[1]{\textcolor{red}{[IMP: #1]}}
\newcommand{\red}[1]{\textcolor{purple}{[#1]}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}



\usepackage{algpseudocode}
% \usepackage[noend,linesnumbered,ruled]{algorithm2e}
\usepackage[vlined,linesnumbered,ruled,algo2e]{algorithm2e}
% \usepackage[algo2e]{algorithm2e} 
% \SetKwProg{Fn}{Function}{}{}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line


% Miscelaneous headers
\usepackage{multicol}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{bm}

\newcommand{\ind}{\perp\!\!\!\!\perp}

% Commands for organizing theorems and proofs

\usepackage{theoremref}
\mathtoolsset{showonlyrefs}

\newtheorem{defn}{Definition}[]
\newtheorem{rem}{Remark}[]
\newtheorem{thm}{Theorem}[]
\newtheorem{claim}{Claim}[]
% \newtheorem{lemma}{Lemma}[]
\newtheorem{prop}{Property}[]
\newtheorem{ass}{Assumption}[]
\newtheorem{cor}{Corollary}[]

% For creating sub-groups of Assumptions/Theorems etc.
\newtheorem{reqm}{Requirement}
% \renewcommand\thereqm{A\arabic{reqm}}

\usepackage{thmtools}
\usepackage{thm-restate}

\declaretheorem[name=Theorem]{rtheorem}
\declaretheorem[name=Proposition]{rproposition}
\declaretheorem[name=Assumption]{rassumption}
\declaretheorem[name=Corollary]{rcorollary}
\declaretheorem[name=Lemma]{rlemma}


% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\pibopt}{\pi_{b^\star}}
\newcommand{\pib}{{\pi_b}}
\newcommand{\pitheta}{{\pi_\btheta}}
\newcommand{\deltheta}{{\frac{\partial}{\partial \btheta}}}
\newcommand{\delthetatwo}{{\frac{\partial^2}{\partial^2 \btheta}}}
\newcommand{\pieval}{{\pi_e}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand{\data}{{\mathcal{D}}}
\newcommand{\ope}{{\operatorname{OPE}}}
\newcommand{\pe}{{\operatorname{PE}}}
\newcommand{\variance}{{\operatorname{Var}}}
\newcommand{\covariance}{{\operatorname{Cov}}}
\newcommand{\bias}{{\operatorname{Bias}}}
\newcommand{\mse}{{\operatorname{MSE}}}
\newcommand{\loss}{{\mathcal{L}}}
\newcommand{\horizon}{{l}}

% Auto sized brackets
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}

\DeclarePairedDelimiter\autobrackett{[}{]}
\newcommand{\brr}[1]{\autobrackett*{#1}}

\DeclarePairedDelimiter\autobrackettt{\{}{\}}
\newcommand{\brrr}[1]{\autobrackettt*{#1}}
